Improving parameter learning of Bayesian nets from incomplete data

This paper addresses the estimation of parameters of a Bayesian network from incomplete data. The task is usually tackled by running the Expectation-Maximization (EM) algorithm several times in order to obtain a high log-likelihood estimate. We argue that choosing the maximum log-likelihood estimate (as well as the maximum penalized log-likelihood and the maximum a posteriori estimate) has severe drawbacks, being affected both by overfitting and model uncertainty. Two ideas are discussed to overcome these issues: a maximum entropy approach and a Bayesian model averaging approach. Both ideas can be easily applied on top of EM, while the entropy idea can be also implemented in a more sophisticated way, through a dedicated non-linear solver. A vast set of experiments shows that these ideas produce significantly better estimates and inferences than the traditional and widely used maximum (penalized) log-likelihood and maximum a posteriori estimates. In particular, if EM is adopted as optimization engine, the model averaging approach is the best performing one; its performance is matched by the entropy approach when implemented using the non-linear solver. The results suggest that the applicability of these ideas is immediate (they are easy to implement and to integrate in currently available inference engines) and that they constitute a better way to learn Bayesian network parameters.

==> bma.tex <==
\subsection{Bayesian Model Averaging}
\label{sec:bma}

A BMA-based approach can also be used to overcome the model uncertainty and overfitting problems. 
The BMA is applied on the alternative estimates returned by the various EM runs in order to obtain a final single estimate.
The rationale is as follows: if we consider as query the variable $X_j$ given its parents, the posterior probability distribution $p(X_j|\pai_j)$ returned by an inference corresponds to the
distribution which is specified in the conditional probability table of the BN for $X_j$.
To answer this query using BMA, we use the estimates identified by each run of EM. We average the returned inferences from models
identified by each EM run, using weights proportional to the score achieved by them.\footnote{Actually, BMA requires to average using as weights the posterior probability of 
each model, obtained as a product of its prior probability and its \textit{marginal} likelihood, which implies in
averaging over the parameters of the models.} %; here we introduce an approximation, using to compute the likelihood a 
%single parameter estimates, namely the one corresponding to the max likelihood.}.
We repeat this query for each $j$ and each combination of $\pai_j$; eventually we instantiate a single BN, by setting $\hat{\theta}_{x_j|\pai_j}=p(x_j|\pai_j)$, 
where $p(x_j|\pai_j)$ is the BMA-averaged inference.
In practice, this can be done by simply averaging the coefficients of the conditional probability tables.
Thus, BMA is \textit{locally} applied to estimate each conditional probability distribution;
we denote as $\hat{\bs{\theta}}$ the estimate obtained in this way.
Note that the inferences returned by $\hat{\bs{\theta}}$ match those produced by the standard BMA 
(which always computes the answer by querying over all the estimated models and then averaging the returned values) 
only for queries on $X_j$ given its parents, and not on more general queries.
However, it is generally not possible to obtain a summary estimate which exactly matches the inferences produced by the standard usage of BMA.
In fact, the standard BMA can be seen as an ensemble of BNs; to get a single estimate, one has to average the joint distributions of these BNs. 
This would produce a representation of the joint probability distribution that is not guaranteed to factorize as the original BN structure. Moreover, it would
be very demanding from the computational viewpoint.
An exception exists for naive structures \cite{dash2002icml}, while our BMA-based approach can be used to estimate the parameters of {\it any} BN.


==> bn3.tex <==
\subsection{Experiments with BN3}
Network BN3 has  structure $A\rightarrow B \rightarrow C$.
We considered two different configurations of number of states for each node: 5-3-5 (meaning $A$,$C$ with 5 categories and $B$ with 3) and 8-4-8 ($A$,$C$ with 8 categories and $B$ with 4). In both cases, we made $B$ randomly missing on 85\% of the instances.  Thus, despite the simple structure of the network, the learning task is interesting since there are many missing data and a moderately high number of states.
The two configurations requires to estimate \textit{from incomplete samples} respectively $2\cdot5+4\cdot3=22$ and $8\cdot3+7\cdot4=52$ parameters; to these numbers, one should add the marginals of $A$, which are however learned from complete samples and whose estimate is thus identical for all methods. 
%%%%%%
We fixed $n$ to 300 for the 5-3-5 configuration and to 500 for the 8-4-8.
%Given the high number of parameters, in this case it was not possible to run the global solver; thus for $C$\_entropy we could only guarantee the  parameter estimates to have a MAP score close enough to that of a local maximum.
In this case, the performance of \textit{C\_entropy} was extremely good. We obtained, for both settings, the following rank in the Friedman test: \textit{1}) \textit{C\_entropy}; \textit{2}) BMA;
\textit{3}) entropy; \textit{4}) MAP. The global MAP was not run, because the number of free unknowns in the continuous optimization problem was too high to achieve
the global solution in reasonable time.
The relative medians for the joint metric are (numbers are given in the order: \textit{C\_entropy}, BMA,  entropy and MAP):
for the 5-3-5 configuration: 0.71, 0.78, 0.90, 1; for the 8-4-8 configuration:
0.68, 0.78, 0.92, 1. These experiments confirm  that, in order to get the most out of the entropy criterion, it is much more effective to have a dedicated solver than applying it on top of  the
multi-start EM. Here, \textit{C\_entropy} is even better than BMA, so its implementation for general settings and further analyses are intended in the near future.
% \begin{figure}
% \begin{centering}
% \includegraphics[width=6cm]{bplot848}
% \par\end{centering}
% \caption{\label{fig:bplot848}Boxplot of  KL-divergences, over 300 data sets ($n$=500) produced by \bnc~in configuration 8-4-8.}
% \end{figure}


==> conclusions.tex <==

\section{Conclusions}

This paper suggests that maximizing (penalized) likelihood or MAP scores is not the best choice to learn the parameters
of a Bayesian network.
In particular, a high score is necessary but not sufficient in order to have a good estimate.
To improve estimation, we propose:
(i) a BMA approach that averages over the estimates learned in different runs of EM,
and (ii) a maximum entropy criterion applied over the estimates with high scores. 
The entropy idea can be implemented on top of EM or using a dedicated non-linear solver, which allows a more fine-grained choice of estimates.
Both BMA and entropy can be promptly integrated into any EM implementation at virtually
no cost in terms of implementation and running time; instead, the non-linear solver for entropy requires some additional implementation effort.
Thorough experiments show that the presented ideas significantly improve the quality of estimates when compared to standard maximum penalized likelihood and MAP ideas.
If EM is used as optimization engine, then BMA yields by far the best results, followed by entropy and MAP.
If the dedicated non-linear solver is used, entropy performs as good as BMA, or even better.
Moreover, for a specific network, we developed a global solver for the MAP estimation. We showed that
its score is only slightly higher than the maximum identified by EM runs, and yet it yields worse estimates. This corroborates
with the other results, indicating that the usual scores do suffer from overfitting and/or model uncertainty.


==> continuous.tex <==
\section{Experiments using Continuous Optimization}\label{sec:contin}
% Our experiments of Section \ref{sec:experiments1} have shown a clear difference in performance among the ideas to
% tackle the model uncertainty, which have put the BMA-based method as the best option against entropy, both superior
% to the standard MAP estimation.
The maximum entropy criterion, applied to the selection of the parameter estimates, 
maximizes entropy while guaranteeing the score to exceed a certain threshold. 
So far, we have applied this idea on top of the multi-start EM, which selects only among estimates returned by the different EM runs.
This approach identifies parameter estimates which are better than those from MAP, but usually worse than BMA's estimates.
An alternative way to implement the idea of maximum entropy is to solve directly the non-linear optimization problem. This requires
to maximize Eq. \eqref{eq:localent} subject to the constraint that the score is only marginally smaller than the best score,
allowing a more fine-grained way to select the estimate than looking at the solutions identified by the different EM runs.
% \hl{Perhaps this sentence can go in Sec. 2.1, together with a discussion of why can we expect the continuous entropy to be better and refs to the paper by schurmans}
This approach is referred in the following as \textit{C\_entropy}. The reason to analyze such situation is that EM runs tend to return local
optima of the score function. However, the maximum entropy estimate might well be a non-optimum estimate in terms of score. Because of that,
even if we increase the number of EM runs and use many more initializations (situation which we have tested), the entropy idea is still confined to saddle points
of the score function, which is only an approximation of a true maximum entropy idea. Therefore, we perform experiments with two specific network structures
with the aim of understanding whether the entropy idea improves by using a continuous optimization method instead of EM.
For ease of expose, we focus only on the joint metric, as this is metric in which entropy is consistently inferior to BMA.


==> intro.tex <==
\section{Introduction}
\label{sec:intro}
This paper focuses on learning the parameters of a Bayesian network
(BN) with \textit{known structure} from incomplete samples, under the assumption of MAR (missing-at-random) missing data.
In this setting, the missing data make the log-likelihood (LL) function  non-concave and multimodal.
% \hl{note: cite EM book to say that penalized EM is EM with prior\\}
The most common approach to maximize LL in the presence of missing data is the Expectation-Maximization (EM) algorithm \cite{dempster1977maximum}, which
generally converges to a local maximum of the LL function.
The EM can be easily modified to maximize, rather than LL, the posterior probability of the data (MAP), as well as other \textit{penalized} maximum likelihood ideas
\cite[Sec 1.6]{mclachlan97}. Generally, maximizing MAP rather than LL yields smoother estimates, less prone to overfitting \cite{lauritzen1995algorithm}.
In the following, we refer to the function to be maximized as the \textit{score}.
Although we focus on
BN learning, the ideas are general and shall apply also to other probabilistic graphical models that share similar characteristics in terms of paramater learning.

In order to reduce the chance of obtaining an estimate with low score,
a multi-start approach is adopted: EM is started from many different initialization points, eventually selecting
the estimate corresponding to the run that achieves the highest score.
We argue however that this strategy has some drawbacks.
% instead better estimates can be selected, by choosing in an alternative way.
%  assuming to adopt a MAP estimation, we refer to this method as 
% % max(MAP).
% we argue however that this is hardly a good decision.
Firstly, the estimate that maximizes the score can well do so because of overfitting. Even if
the MAP estimation is adopted, the fixed structure and the amount of data may lead to overfitting, because they might not
fully represent the distribution that generated the data.
Secondly, the estimates produced by the different EM runs are typically very different from each other, and yet achieve
very close scores \cite[Chap. 19]{koller2009probabilistic}.
Choosing the single estimate with highest score implies in \textit{model uncertainty}, because the estimates with slightly worse score are completely ignored.
Overall, the score alone does not seem to be powerful enough to identify the best estimate.
Note that the challenge presented here does not involve model complexity: all the competing estimates have the
same underlying structure and thus approaches such as the Bayesian Information Criterion (BIC) do not apply.
% as they would choose the estimates which maximize the score.

We propose and compare two approaches to replace the criterion of selecting the highest score estimate, both based on well-known ideas already applied in other contexts.
The first is based on the principle of maximum entropy and the second on model averaging.
The maximum entropy criterion  can be stated as:
''\textit{when we make inferences on incomplete information, we should draw them from that probability distribution that has the maximum entropy permitted by the information which we do have}``
\cite{jaynes82}. We interpret this principle
by first discarding estimates with low score, which we assume to be poor, and then by selecting the most entropic estimate among the remaining ones. 
The entropy-based criterion is expected to yield parameter estimates that are more robust to overfitting than those from the criterion of maximum score.
In its simplest version, we apply the entropy principle on top of a multi-start EM; in a more sophisticated fashion, we implement it using a non-linear solver.
In \cite{wang05ml}, a similar idea has been explored  to fit
continuous distributions from only partial knowledge about moments or other features that are extracted from data.
% In this
% % situation, the principle states that one should choose the distribution that is maximally uninformative with regard to missing information; thus, we choose the distribution that has maximal entropy subject to any informative constraint we can justify. 
%
% The former searches for the most conservative estimate among
% those estimates of high score, while the latter resembles Bayesian model averaging.
% The goal of this paper is to compare  these ideas to best select the parameter estimate for learning a BN from incomplete data.
%
% As already mentioned, different parameter estimates yield similar scores, despite being (even strongly) different.
% Choosing the estimate of highest score can be criticized not only for possible overfitting, but also because it overlooks \textit{model uncertainty}.
% Usually several discarded estimates have a score which is barely smaller than that of the selected one, still all
% subsequent inferences are going to be performed on the basis of the single selected model,
% completely ignoring the discarded ones.
The model averaging idea is instead  inspired by Bayesian Model Averaging (BMA, see \cite{hoeting1999bayesian}),
and is designed to be used on top of the multi-start EM.
BMA is  a technique specifically  designed to deal with
model uncertainty, which prescribes to average the predictions produced by a set of competing
models, assigning to each model a weight proportional to its posterior
probability. %It is thus based on a collection of competing models.
In the literature, BMA has been often used to manage ensembles of BN classifiers; yet, most attempts
were not successful, as reviewed by \cite{cerquides2005robust}.
The problem is that a single model becomes usually much more probable than any competitor, and thus there is little difference
between using BMA or the single most probable model (that is, the maximum score one). 
%One can see the estimates generated by the different EM runs as competing models with close scores; this
%could prevent BMA from  getting sharply peaked around a single model.
Our approach is to apply BMA locally to each conditional probability distribution that defines the BN; this allows us to instantiate a single BN model, whose parameters can be readily inspected,
instead of dealing with a collection of models.
% This could be welcome in applications where the domain experts look for insights from the parameter estimates.
%\begin{itemize}
% \item \hl{it is known that max(LL) does not work; although MAP is a way to reduce, max(MAP) is still not enough; entropy and BMA are possible solutions}
%\item \hl{we compare EM+entropy, EM+BMA, both are expected to be better than EM+max(MAP), because .... }
%\item \hl{EM+BMA works better than EM+entropy, and both of them are considerably better than EM+max(MAP)}
%\item \hl {to get the maximum out of entropy, we need the analytical solver, which allows the parameter estimate to not correspond to a
%local maximum of LL; experiments with simple networks are very promising}
%\end{itemize}

Sections \ref{sec:expe} and  \ref{sec:contin} present a vast amount of experiments with different BNs and missingness processes.
% We use three distinct real-world structures and a large set of random generated structures and parameters.
These experiments, performed on a grid of computers, would have taken more than nine months if run on a single desktop computer.
% The comparison is based on the KL divergence of the estimate to the true distribution, on the KL divergence of the most connected 
% query node given its Markov blanket (which simulates a regression/classification problem), and on the KL divergence of the marginal
% distribution of all the leaves. This latter case is used to demonstrate that the advantage of BMA and entropy of the standard highest
% scoring approach reduces when most of the variables of the network are summed out, as expected. Overall,
They consistently show that both  the entropy and the BMA-based approaches provide better estimates than
the maximum score estimation, and that these better parameters also result in better inferences with the resulting BNs.
% If multi-start EM is to be adopted to maximize the score, then the BMA-based approach yields the best parameter estimates and inferences; those performance 
% is only matched  by the entropy idea, when implemented using continuous optimization, which thus requires the effort of developing a dedicated solver.

% the results indicate that the estimates based solely on the score function, even if globally optimized, are inferior to those obtained
% by both the BMA and the entropy ideas. Moreover, BMA is superior to entropy when used on top an EM method. I
% n order to understand
% better this distinction, we have also run the entropy idea n this case, the entropy-based method
% improves with respect to the version on top of EM, and achieves results that are comparable to those of BMA.
%The novel methods (entropy, empirical entropy and BMA) considerably
%outperform, in terms of KL divergence, the standard approach of retaining the parameterization with highest score.
%BMA and entropy provide best performance, followed by empirical entropy.


